Is Your Large Language Model Knowledgeable or a Choices-Only Cheater?

Recent work shows that large language models (LLMs) can answer multiple-choice questions using only the choices, but does this mean that MCQA leaderboard rankings of LLMs are largely influenced by abilities in choices-only settings? To answer this, we use a contrast set that probes if LLMs over-rely on choices-only shortcuts in MCQA. While previous works build contrast sets via expensive human annotations or model-generated data which can be biased, we employ graph mining to extract contrast sets from existing MCQA datasets. We use our method on UnifiedQA, a group of six commonsense reasoning datasets with high choices-only accuracy, to build an 820-question contrast set. After validating our contrast set, we test 12 LLMs, finding that these models do not exhibit reliance on choice-only shortcuts when given both the question and choices. Thus, despite the susceptibility~of MCQA to high choices-only accuracy, we argue that LLMs are not obtaining high ranks on MCQA leaderboards just due to their ability to exploit choices-only shortcuts.

==> data/quant_adv.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{data/benchmark_adv.png}
    \vspace{-4.5ex}
    \caption{Our modified LLaMA-70B and Gemma-2B accuracy on the full evaluation set and its contrast set.}
    \label{fig:adv}
    \vspace{-2ex}
\end{figure}
